Higher Gauge Theory

This is an invited survey article on higher gauge theory for the Encyclopedia of Mathematical Physics, 2nd edition. In particular, we provide a lightning introduction to higher structures and to the construction of the kinematical data of higher gauge theories, i.e. connections on higher principal bundles. We also summarise the most important applications and dynamical principles that have appeared in the literature, and we close with comments on related areas.

==> lib/characters.tex <==
\newcommand{\makecommand}[3]{%
	\foreach \i in #3 {%
    	\expandafter\xdef\csname #1\i\endcsname{{\noexpand#2{\unexpanded\expandafter{\i}}}}%
  	}%
}

%
% Characters
%

\newcommand{\latinalphabet}{A,a,B,b,C,c,d,D,E,e,F,f,G,g,H,h,I,i,J,j,K,k,L,l,M,m,N,n,O,o,P,p,Q,q,R,r,S,s,T,t,U,u,V,v,W,w,X,x,Y,y,Z,z}
\newcommand{\Latinalphabet}{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\makecommand{I}{\mathbbm}{\latinalphabet}
\makecommand{bf}{\mathbf}{\latinalphabet}
\makecommand{bm}{\bm}{\latinalphabet}
\makecommand{ca}{\mathcal}{\Latinalphabet}
\makecommand{fr}{\mathfrak}{\latinalphabet}
\makecommand{rm}{\mathrm}{\latinalphabet}
\makecommand{sf}{\mathsf}{\latinalphabet}
\makecommand{sc}{\mathscr}{\latinalphabet}
\makecommand{tt}{\mathtt}{\latinalphabet}

\makecommand{bar}{\bar}{\latinalphabet}
\makecommand{dot}{\dot}{\latinalphabet}

\newcommand{\eps}{\varepsilon}

%
% Lie groups and algebras
%

\makecommand{sf}{\mathsf}{{GL,SL,O,SO,OSp,U,SU,Sp,Spin,String}}
\makecommand{fr}{\mathfrak}{{Lie,gl,sl,o,so,osp,u,su,sp,spin,string}}

%
% Categories, operads, etc.
%

\makecommand{Cat}{\mathsf}{{Ass,Bibun,Cart,Cat,Com,DiffCat,End,Fun,GradSMod,GradVect,Grp,Grpd,Lie,Mfd,Oper,poSet,Schur,SMod,Set,SMfd,sGrp,sMfd,sSet,sSh,sSMfd,SurSub,Top,Vect,VectBun}}

\makecommand{sf}{\mathsf}{{Bun,CE,Ch,Dec,Der,Diag,End,Hom,hom,inthom,Jet,Kan,TDiff}}

\newcommand{\opEnd}{{{\caE}nd}}
\newcommand{\OpEnd}{{{\scE}\!nd}}
\newcommand{\opCom}{{{\caC}om}}
\newcommand{\OpCom}{{{\scC}\!om}}
\newcommand{\opAss}{{{\caA}ss}}
\newcommand{\OpAss}{{{\scA}\!ss}}
\newcommand{\opLie}{{{\caL}ie}}
\newcommand{\OpLie}{{{\scL}\!ie}}
\newcommand{\opGer}{{{\caG}er}}
\newcommand{\OpGer}{{{\scG}\!er}}
\newcommand{\opBV}{{{\caB\caV}}}
\newcommand{\OpBV}{{{\scB\scV}}}
\newcommand{\opqBV}{{q{\caB\caV}}}
\newcommand{\OpqBV}{{q{\scB\scV}}}
\newcommand{\opDual}{{{\caD}ual}}
\newcommand{\OpDual}{{{\scD}\!ual}}
\newcommand{\opGam}{{{\caG}am}}
\newcommand{\OpGam}{{{\caG}\!am}}
\newcommand{\opHom}{{{\caH}om}}
\newcommand{\OpHom}{{{\caH}\!om}}

==> lib/commands.tex <==
%
% Arrows
%

\newcommand{\multirightarrow}[1]{%
	\mathrel{%
		\substack{%
			\let\multiarrowcontent\empty
			\foreach \i in {1,...,#1} {
	    		\ifnum\i=#1
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longrightarrow}
	    		\else
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longrightarrow\\[-0.6ex]}
	    		\fi
			} 
			\multiarrowcontent%
		}%
	}%
}

\newcommand{\multileftarrow}[1]{%
	\mathrel{%
		\substack{%
			\let\multiarrowcontent\empty
			\foreach \i in {1,...,#1} {
	    		\ifnum\i=#1
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longleftarrow}
	    		\else
	    			\expandafter\gappto\expandafter\multiarrowcontent\expandafter{\longleftarrow\\[-0.6ex]}
	    		\fi
			} 
			\multiarrowcontent%
		}%
	}%
}

\renewcommand{\twoheadrightarrow}{\mathrel{\mathrlap{\rightarrow}\mkern.5mu\rightarrow}}
\DeclareRobustCommand\longtwoheadrightarrow{\relbar\joinrel\twoheadrightarrow}
\renewcommand{\twoheadleftarrow}{\mathrel{\mathrlap{\leftarrow}\mkern.5mu\leftarrow}}
\DeclareRobustCommand\longtwoheadleftarrow{\twoheadleftarrow\joinrel\relbar}

%
% Derivatives
%

\newcommand{\dder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\mathrm{d}}{\mathrm{d} #2}%
	}{%
		\frac{\mathrm{d} #1}{\mathrm{d} #2}%
	}%
}
\newcommand{\parder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\partial}{\partial #2}%
	}{%
		\frac{\partial #1}{\partial #2}%
	}%
}
\newcommand{\delder}[2][]{%
	\ifthenelse{\equal{#1}{}}{%
		\frac{\delta}{\delta #2}%
	}{%
		\frac{\delta #1}{\delta #2}%
	}%
}

%
% Inner products
%

\newcommand{\inner}[2]{\langle#1,#2\rangle}
\newcommand{\innerLarge}[2]{\left\langle#1,#2\right\rangle}

%
% Vectors
%

\newcommand{\colvec}[1]{%
    \begingroup
        \newcommand\listcontent{}
        \def\do##1{\appto\listcontent{##1\\}}
        \expandafter\docsvlist\expandafter{#1}
        \begin{pmatrix}
            \listcontent
        \end{pmatrix}
    \endgroup
}

%
% Integrals
%

\DeclareMathOperator*{\sumint}{%
\mathchoice%
	{\ooalign{$\displaystyle\sum$\cr\hidewidth$\displaystyle\int$\hidewidth\cr}}
	{\ooalign{\raisebox{.14\height}{\scalebox{.7}{$\textstyle\sum$}}\cr\hidewidth$\textstyle\int$\hidewidth\cr}}
	{\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
	{\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
}

\DeclareMathOperator*{\cpv}{\setbox0=\hbox{$\int$}\int\hskip-\wd0{}\hskip-\wd0{~-~}} % Cauchy principal value

%
% Miscellaneous
%

\newcommand\acton{\mathbin\vartriangleright} % action
\DeclareMathOperator{\Ad}{Ad} % adjoint map
\DeclareMathOperator{\ad}{ad} % adjoint map
\DeclareMathSymbol{\antishriek}{\mathord}{operators}{'74} %antishriek
\DeclareMathOperator{\coker}{coker} % cokernel
\DeclareMathOperator{\diag}{diag} % diagonal matrix
\DeclareMathOperator{\lvac}{\langle 0|} % vacuum
\DeclareMathOperator{\id}{\mathrm{id}} % identity
\DeclareMathOperator{\sfid}{\mathsf{id}} % identity
\DeclareMathOperator{\im}{im} % image
\newcommand{\normal}[1]{\mathop{:\mathrel{#1}:}} % normal ordering
\DeclareMathOperator{\pr}{\mathsf{pr}} % projection
\newcommand{\spacer}[1]{\vrule width0pt height0pt depth#1\relax}
\DeclareMathOperator{\spn}{span} % span
\DeclareMathOperator{\str}{str} % super trace
\newcommand{\tocut}[1]{{\color{green} #1 }}
\newcommand{\todo}[1]{{\color{red} #1 }}
\DeclareMathOperator{\tr}{tr} % trace
\DeclareMathOperator{\rvac}{|0\rangle} % vacuum
%\newcommand{\uline}[1]{\ul{\itshape #1}}
\newcommand{\uline}[1]{\ul{\emph{#1}}}
\DeclareMathOperator{\unit}{\mathbbm{1}} % unit matrix
\DeclareMathOperator{\lap}{\mathop\Delta\nolimits} % Laplacian
\DeclareMathOperator{\wave}{{\mathop\oldsquare\nolimits}} % adjust sup/subscripts for the d'Alembertian
\DeclareMathOperator{\intprod}{\mathbin{\raisebox{\depth}{\scalebox{1}[-1]{$\lnot$}}}} % interior product

%
% Prepositions
%

\newcommand{\efor}{{~~~\mbox{for}~~~}}
\newcommand{\eforall}{{~~~\mbox{for all}~~~}}
\newcommand{\eand}{{~~~\mbox{and}~~~}}
\newcommand{\eelse}{{~~~\mbox{else}~~~}}
\newcommand{\eon}{{~~~\mbox{on}~~~}}
\newcommand{\eor}{{~~~\mbox{or}~~~}}  		
\newcommand{\ewith}{{~~~\mbox{with}~~~}}

%
% Young diagrams
%

\newcommand{\tyng}[1]{\hbox{\tiny$\yng #1$}} % small Young diagram
\newcommand{\tyoung}[1]{\hbox{\tiny$\young #1$}} % small Young diagram


==> lib/hyphenation.tex <==
\hyphenation{mani-folds mani-fold opera-tor bet-ween}
